A Control Theoretic Framework for Adaptive Gradient Optimizers in Machine Learning

Adaptive gradient methods have become popular in optimizing deep neural networks; recent examples include AdaGrad and Adam. Although Adam usually converges faster, variations of Adam, for instance, the AdaBelief algorithm, have been proposed to enhance Adam's poor generalization ability compared to the classical stochastic gradient method. This paper develops a generic framework for adaptive gradient methods that solve non-convex optimization problems. We first model the adaptive gradient methods in a state-space framework, which allows us to present simpler convergence proofs of adaptive optimizers such as AdaGrad, Adam, and AdaBelief. We then utilize the transfer function paradigm from classical control theory to propose a new variant of Adam, coined AdamSSM. We add an appropriate pole-zero pair in the transfer function from squared gradients to the second moment estimate. We prove the convergence of the proposed AdamSSM algorithm. Applications on benchmark machine learning tasks of image classification using CNN architectures and language modeling using LSTM architecture demonstrate that the AdamSSM algorithm improves the gap between generalization accuracy and faster convergence than the recent adaptive gradient methods.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}




\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{See Section~\ref{sec:intro} and Section~\ref{sec:summary}.}
  \item Did you describe the limitations of your work?
    \answerYes{See Section~\ref{sec:summary}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{There is no foreseeable negative impacts of this work.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{See Section~\ref{sec:adagrad} and Section~\ref{sec:gen}.}
  \item Did you include complete proofs of all theoretical results?
    \answerYes{See the supplemental material.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{sec:exp} and supplemental material.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:exp} and supplemental material.}
    \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Qualitative comparison between the algorithms was consistent over multiple runs.}
    \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{The experiments were executed in a personal computer with Intel(R) Core(TM) i7-10750H CPU @ 2.6 GHz, 64 bit OS, i915 Intel GFX Driver, and NVIDIA GeForce GTX 2070 with Max-Q Design. }
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{See the References.}
  \item Did you mention the license of the assets?
    \answerNA{We have only used published assets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{We have only used published assets.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{The datasets used in this work do not contain any personally identifiable information or offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> general.tex <==
\section{A Generic Adaptive Gradient Algorithm}
\label{sec:gen}

In this section, we propose a generic adaptive gradient algorithm and create a state-space framework for analyzing Adam-like adaptive gradient algorithms. 
% and inspired by the analysis of G-AdaGrad algorithm, as presented in the proof of Theorem~\ref{thm:adagrad}.

We make the following assumptions in order to present the algorithms in this paper and their convergence results.

\begin{assumption} \label{assump_1}
Assume that the minimum of function $f$ exists and is finite, i.e., $\mnorm{\min_{x \in \R^d} f(x)} < \infty$.
\end{assumption}

\begin{assumption} \label{assump_2}
Assume that $f$ is twice differentiable over its domain $\R^d$ and the entries in the Hessian matrix $\nabla^2 f(x)$ are bounded for all $x\in \R^d$.
\end{assumption}

The above assumptions are mild and standard in the literature of gradient-based optimization. Assumption~\ref{assump_1} implies that the optimization problem~\eqref{eqn:opt_1} has a solution. Assumption~\ref{assump_2} is equivalent to the gradient $\nabla f$ being Lipschitz continuous, which is also referred as the function $f$ being {\em smooth}~\cite{ZaheerRSKK18, de2018convergence}.

Our framework of adaptive gradient algorithms hinges on their state-space representation in terms of ODEs. The proposed generic adaptive gradient algorithm is similar to the Adam method described in Section~\ref{sub:adam}. However, there are two notable differences.
\begin{itemize}
    \item Firstly, we replace the squared-gradient term $\norm{\nabla_i f(x(t))}^2$ in the evolution of second raw moment estimate in~\eqref{eqn:v_adam} with $\psi(\nabla_i f(x(t)), \mu_i(t))$, where we define $\psi$ as an well-behaved and non-negative valued function $\psi:\R^2 \to \R_{\geq 0}$. The sufficient conditions on the general function $\psi$ which guarantees convergence of the generic algorithm are specified later in this section. Needless to say, the generic setup includes the original Adam algorithm, i.e., $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$, as a special case.
    \item The other difference is that, in our algorithm, the ODE governing the second raw moment estimate of the gradients has a higher order. An issue with the Adam algorithm is that the ODEs~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} for the first and second moments can converge slowly, especially if the optimization problem~\eqref{eqn:opt_1} is ill-conditioned, leading to a slower convergence of the estimate. Now, each of the ODEs~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} can be seen as a controlled linear-time invariant (LTI) system. The controlled inputs for~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} are, respectively, $\nabla_i f(x(t))$ and $\norm{\nabla_i f(x(t))}^2$. It is known that addition of a zero improves the transient response of an LTI system. Note that, the Adam algorithm does not have any zero in the dynamics~\eqref{eqn:v_adam}. So, in our algorithm, we add a left-half plane zero to the dynamics in~\eqref{eqn:v_adam} for improving the convergence rate. However, in the Adam algorithm, the dynamics in~\eqref{eqn:v_adam} is {\em strictly proper}. Thus, we also add an additional left half-plane pole in~\eqref{eqn:v_adam}. Hence, for each dimension $i \in \{1,\ldots,d\}$, the transfer function from $\psi(\nabla_i f(x(t)), \mu_i(t))$ to the second raw moment estimate $\nu_i(t)$ in our generic setup has an additional pole-zero pair in the left-half plane, as compared to only one pole and no zero for its counterpart in the Adam method. Herein lies the intuition behind our algorithm.
\end{itemize}

% We demonstrate this with the following numerical example. In this example, we consider the classification task of handwritten digits one and five, using the MNIST~\cite{} dataset. We consider the logistic regression model and conduct experiments for minimizing the cross-entropy error on the training data. 

Our generic adaptive gradient algorithm is iterative in nature where, at each time $t\geq 1$, it maintains four $d$-dimensional vectors: an estimate $x(t)$ of a minimum point of~\eqref{eqn:opt_1}, an estimate $\mu(t)$ of the first moment of gradients, an estimate $\nu(t)$ of the second raw moment of gradients, and an additional $\zeta(t)$ due to higher order of the transfer functions from $\psi(\nabla_i f(x(t)), \mu_i(t))$ to $\nu_i(t)$. The initial estimate $x(1)$ is chosen arbitrarily from $\R^d$. The variables $\mu$ and $\zeta$ are initialized at $t=1$ as the $d$-dimensional zero vector, denoted by $0_d$. The remaining variable $\nu$ is initialized according to $\{\nu_i(1) > 0 : i = 1,\ldots,d\}$. Before initiating the iterative process, the algorithm chooses three real-valued scalar parameters $\lambda_1$, $\lambda_2$, and $\lambda_3$, each within the interval $(0,1)$. Their specific values are presented later in this section. Recall the definition of the function $\alpha: [1,\infty) \to \R$ from~\eqref{eqn:alpha}. For each time $t\geq 1$, the algorithm steps in continuous-time domain are governed by the following set of ODEs
\begin{align}
    \Dot{\mu}_i(t) & = -\lambda_1 \mu_i(t) + \lambda_1 \nabla_i f(x(t)), \label{eqn:mu_evol} \\
    \Dot{\zeta}_i(t) & = -\lambda_2 \zeta_i(t) + \lambda_2 \nu_i(t), \label{eqn:z_evol} \\
    \Dot{\nu}_i(t) & = \lambda_3 \zeta_i(t) - (\lambda_2 + \lambda_3) \nu_i(t) + \lambda_2 \psi(\nabla_i f(x(t)), \mu_i(t)), \label{eqn:nu_evol} \\
    \Dot{x}_i(t) & = - \dfrac{1}{\alpha(t)} \dfrac{\mu_i(t)}{\sqrt{\nu_i(t)}}. \label{eqn:xm_evol}
\end{align}
The $d$-dimensional vectors $\mu$, $\zeta$, and $\nu$ can be abstracted as dynamic controller states.

\begin{assumption} \label{assump_3}
We assume that the function $\psi$ satisfies the following properties.
\begin{enumerate}[label={\textbf{\Alph*:}},
  ref={\theassumption.\Alph*}]
    \item $\psi$ is differentiable over $\R^2$. Moreover, $\psi(x,y)$ and its gradient $\nabla \psi (x,y)$ are bounded if both $x$ and $y$ are bounded, for any $x,y \in \R$. \label{assump_a}
    \item $\psi(x,.)$ is bounded only if $x$ is bounded, for $x \in \R$. \label{assump_b}
    \item $\lim_{t \to \infty} \psi(\nabla_i f(x(t)), \mu_i(t)) = 0$ only if $\lim_{t \to \infty} \nabla_i f(x(t)) = 0$. \label{assump_c}
\end{enumerate}
\end{assumption}

Assumption~\ref{assump_a} implies that the function $\psi$ is smooth enough. Assumption~\ref{assump_b} means that $\psi$ is radially unbounded in its first argument.

The following theorem guarantees convergence of our generic adaptive gradient algorithm, presented above in~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol}, to a critical point of problem~\eqref{eqn:opt_1}.

\begin{theorem} \label{thm:gen}
Consider the set of differential equations~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with initial conditions $\mu(1) = \zeta(1) = 0_d$, $x(1) \in \R^d$, and $\{v_i(1) > 0 : i = 1,\ldots,d\}$. Let the parameters $\lambda_1$, $\lambda_2$ and $\lambda_3$ satisfy
\begin{align}
    0 < \lambda_2 < \lambda_1 < 1, \, \lambda_3 \geq 0, \, \lambda_2 + \lambda_3 < 4\lambda_1. \label{eqn:lambda_cond}
\end{align}
If Assumptions~\ref{assump_1}-\ref{assump_3} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{theorem}


\begin{proof}
The time-derivative of $f$ along the trajectories $x(t)$  of~\eqref{eqn:xm_evol} is given by
\begin{align}
    \Dot{f}(x(t)) &= \sum_{i=1}^d \nabla_i f(x(t)) \Dot{x}_{i}(t) = - \sum_{i=1}^d \dfrac{\nabla_i f(x(t))}{\alpha(t)} \dfrac{\mu_i(t)}{\sqrt{\nu_i(t)}}. \label{eqn:fdot_2}
\end{align}
Multiplying with $\alpha(t)$ on both sides above we get
\begin{align*}
    \alpha(t)\Dot{f}(x(t)) = - \sum_{i=1}^d \nabla_i f(x(t)) \dfrac{\mu_i(t)}{\sqrt{\nu_i(t)}}.
\end{align*}
Upon integrating both sides above w.r.t. $s$ from $1$ to $t$ and substituting from~\eqref{eqn:mu_evol} we have
\begin{align}
    & \int_1^t \alpha(s)\Dot{f}(x(s))ds = - \sum_{i=1}^d \int_1^t \dfrac{(\Dot{\mu}_i(s) + \lambda_1 \mu_i(s)) \mu_i(s)}{\lambda_1 \sqrt{\nu_i(s)}}ds \nonumber\\
    &= - \sum_{i=1}^d \int_1^t \dfrac{\mu_i(s)\Dot{\mu}_i(s)}{\lambda_1 \sqrt{\nu_i(s)}}ds - \sum_{i=1}^d \int_1^t \dfrac{\mu_i(s)^2}{\sqrt{\nu_i(s)}}ds. \label{eqn:total_int}
\end{align}
Integrating by parts we have the first term on R.H.S. as
\begin{align*}
    & \int_1^t \dfrac{\mu_i(s)\Dot{\mu}_i(s)}{\sqrt{\nu_i(s)}}ds
    = \left[\dfrac{\mu_i(s)^2}{2\sqrt{\nu_i(s)}}\right]_1^t + \dfrac{1}{4} \int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \Dot{\nu}_i(s) ds.
\end{align*}
Upon substituting above from~\eqref{eqn:nu_evol}, and using that $\mu(1)=0_d$ we have
\begin{align*}
    & \int_1^t \dfrac{\mu_i(s)\Dot{\mu}_i(s)}{\sqrt{\nu_i(s)}}ds
    = \dfrac{\mu_i(t)^2}{2\sqrt{\nu_i(t)}} + \dfrac{\lambda_3}{4} \int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \\
    & - \dfrac{\lambda_2+\lambda_3}{4}\int_1^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \\
    & + \dfrac{\lambda_2}{4}\int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds.
\end{align*}
Upon substituting above in~\eqref{eqn:total_int} we obtain that
\begin{align}
    & \int_1^t \alpha(s)\Dot{f}(x(s))ds
    = - \sum_{i=1}^d \dfrac{\mu_i(t)^2}{2\lambda_1\sqrt{\nu_i(t)}} \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_3}{4\lambda_1} \int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \nonumber \\
    & - \sum_{i=1}^d \left(1-\dfrac{\lambda_2+\lambda_3}{4\lambda_1}\right)\int_1^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_2}{4\lambda_1}\int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds. \label{eqn:int_expand}
\end{align}

We define, $\gamma_1 = 1-\lambda_1$ and $\gamma_2 = 1-\lambda_2$.
Upon differentiating both sides of~\eqref{eqn:alpha} w.r.t $t$ we get $\Dot{\alpha}(t) = \dfrac{\gamma_2^t(1-\gamma_1^t)\log{\gamma_2} - 2\gamma_1^t(1-\gamma_2^t)\log{\gamma_1}}{2(1-\gamma_2^t)^{1.5}}$.
So we have
\begin{align}
    \Dot{\alpha}(t) < 0 \iff \left(\dfrac{\gamma_2}{\gamma_1}\right)^t \dfrac{1-\gamma_1^t}{1-\gamma_2^t} > 2\dfrac{\log{\gamma_1}}{\log{\gamma_2}}. \label{eqn:cond}
\end{align}
From the condition $\lambda_1 > \lambda_2$ in~\eqref{eqn:lambda_cond}, we have $1 > \gamma_2 > \gamma_1 > 0$. Then, $\left(\dfrac{\gamma_2}{\gamma_1}\right)^t$ and $\dfrac{1-\gamma_1^t}{1-\gamma_2^t}$ are, respectively, increasing and decreasing functions of $t$. Since $1 > \gamma_2 > \gamma_1 > 0$, we have $\lim_{t \to \infty} \left(\dfrac{\gamma_2}{\gamma_1}\right)^t \to \infty$ and $\lim_{t \to \infty} \dfrac{1-\gamma_1^t}{1-\gamma_2^t} = 1$. Thus, $\left(\dfrac{\gamma_2}{\gamma_1}\right)^t \dfrac{1-\gamma_1^t}{1-\gamma_2^t}$ is an increasing function of $t$. Then, there exists $T < \infty$ such that~\eqref{eqn:cond} holds for all $t \geq T$. 
Integrating by parts we rewrite the L.H.S. in~\eqref{eqn:int_expand} as
\begin{align*}
    & \int_1^t \alpha(s)\Dot{f}(x(s))ds = \left[\alpha(s)f(x(s))\right]_1^t - \int_1^t \Dot{\alpha}(s)f(x(s))ds.
\end{align*}
Upon substituting from above in~\eqref{eqn:int_expand}, for $t \geq T$,
\begin{align}
    & \alpha(t)f(x(t)) + \sum_{i=1}^d \dfrac{\mu_i(t)^2}{2\lambda_1\sqrt{\nu_i(t)}} = \alpha(1)f(x(1)) \nonumber \\
    & + \int_1^{T} \Dot{\alpha}(s)f(x(s))ds + \int_{T}^t \Dot{\alpha}(s)f(x(s))ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_3}{4\lambda_1} \int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \nonumber \\
    & - \sum_{i=1}^d \left(1-\dfrac{\lambda_2+\lambda_3}{4\lambda_1}\right)\int_1^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_2}{4\lambda_1}\int_1^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds. \label{eqn:alphaV}
\end{align}

For each $i \in \{1,\ldots,d\}$, consider the LTI system described by~\eqref{eqn:z_evol}-\eqref{eqn:nu_evol}, with the state vector $[\zeta_i,\nu_i]^T \in \R^2$. From~\eqref{eqn:lambda_cond}, $\lambda_3 \geq 0$. Here, we consider the possible cases: $\lambda_3 > 0$ and $\lambda_3 = 0$.
\begin{itemize}
    \item $\lambda_3 > 0$ : Define the state matrix $A = \begin{bmatrix} -\lambda_2 & \lambda_2 \\ \lambda_3 & -(\lambda_2+\lambda_3) \end{bmatrix}$. Since $\zeta(1) = 0_d$, the states are given by the solution
\begin{align*}
    \begin{bmatrix} \zeta_i(t) \\ \nu_i(t) \end{bmatrix} & = e^{A (t-1)} \begin{bmatrix} 0 \\ \nu_i(1)\end{bmatrix} \\ & + \int_1^t e^{A (t-s)} \begin{bmatrix} 0 \\ \lambda_2 \end{bmatrix} \psi(\nabla_i f(x(s)), \mu_i(s)) d s.
\end{align*}
Upon computing the state-transition matrix $e^{A t}$ and substituting above, we obtain that
\begin{align}
    \zeta_i(t) & = \phi_{12}(t-1) \nu_i(1) \nonumber \\ & + \lambda_2 \int_1^t \phi_{12}(t-s) \psi(\nabla_i f(x(s)), \mu_i(s)) d s, \label{eqn:zt} \\
    \nu_i(t) & = \phi_{22}(t-1) \nu_i(1) \nonumber \\ & + \lambda_2 \int_1^t \phi_{22}(t-s) \psi(\nabla_i f(x(s)), \mu_i(s)) d s, \label{eqn:nut}
\end{align}
where $\phi_{12}(t) = \lambda_2 e^{-\frac{2\lambda_2+\lambda_3}{2}t} \frac{e^{\frac{p}{2}t}-e^{-\frac{p}{2}t}}{p}$, $\phi_{22}(t) = e^{-\frac{2\lambda_2+\lambda_3}{2}t} \frac{e^{\frac{p}{2}t}(p-\lambda_3) + e^{-\frac{p}{2}t}(p+\lambda_3)}{2p}$, and $p = \sqrt{\lambda_3^2 + 4\lambda_2\lambda_3}$. Since $\lambda_2 > 0$ (ref.~\eqref{eqn:lambda_cond}), $\nu_i(1) > 0$, $\psi \geq 0$, and $p > 0$, from~\eqref{eqn:zt} we have $\zeta_i(t) > 0$. Since $\lambda_2, \lambda_3 > 0$, we have $p = \sqrt{\lambda_3^2 + 4\lambda_2\lambda_3} > \lambda_3$, which implies that $\phi_{22}(t) > 0$. From above and $\nu_i(1) > 0$, we have $\nu_i(t) > 0$.
    \item $\lambda_3 = 0$ : From~\eqref{eqn:nu_evol}, $\Dot{\nu}_i(t) = - \lambda_2 \nu_i(t) + \lambda_2 \psi(\nabla_i f(x(t)), \mu_i(t))$. The solution of this ODE is $\nu_i(t) = e^{-\lambda_2 (t-1)} \nu_i(1) + \lambda_2 \int_1^t e^{-\lambda_2 (t-s)} \psi(\nabla_i f(x(s)), \mu_i(s)) d s$, which implies that $\nu_i(t) > 0$.
\end{itemize}

Since $\zeta_i(t) > 0$ and $\psi \geq 0$, due to~\eqref{eqn:lambda_cond} and~\eqref{eqn:cond}, the R.H.S. in~\eqref{eqn:alphaV} is decreasing in $t \geq T$. Then, the L.H.S. in~\eqref{eqn:alphaV} is also decreasing in $t \geq T$. Since $\mu_i(t)$ and $\nu_i(t)$ are continuous and $\nu_i(t) > 0$, $\dfrac{\mu_i(t)^2}{2\lambda_1\sqrt{\nu_i(t)}}$ is continuous. Also, $\alpha(t)f(x(t))$ is continuous. Thus, considering the compact interval $[1,T]$, $\alpha(T)f(x(T)) + \sum_{i=1}^d \dfrac{\mu_i(T)^2}{2\lambda_1\sqrt{\nu_i(T)}} =: M_T$ is finite. Since the L.H.S. in~\eqref{eqn:alphaV} is decreasing in $t \geq T$, we have the L.H.S. in~\eqref{eqn:alphaV} bounded above by $M_T$ for all $t \geq T$. 

From the R.H.S. of~\eqref{eqn:alphaV} then we have that $\mu_i(t)^2 \nu_i(t)^{-1.5} \psi(\nabla_i f(x(t)), \mu_i(t))$ and $\mu_i(t)^2 \nu_i(t)^{-0.5}$ are integrable w.r.t. $t$ and bounded. Thus, $\mu_i(t)$ is bounded. It implies that, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded unless $\mu_i(t) = 0$ or $\nu_i(t) = \infty$. From~\eqref{eqn:xm_evol}, either of the conditions $\mu_i(t) = 0$ and $\nu_i(t) = \infty$ implies that $\dot{x}_i(t) = 0$ and, hence, $\frac{d}{dt}\nabla_i f(x(t)) = 0$. Due to continuity of $\nabla_i f$, we then have $\nabla_i f(x(t))$ is bounded. From Assumption~\ref{assump_a}, $\nabla_i f(x(t))$ and $\mu_i(t)$ being bounded implies that $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded, if $\mu_i(t) = 0$ or $\nu_i(t) = \infty$. Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded, and therefore, Assumption~\ref{assump_b} implies that $\nabla_i f(x(t))$ is bounded. 

% Integrating both sides of~\eqref{eqn:mu_evol} w.r.t $t$ from $1$ to $t$, we have for $i \in \{1,\ldots,d\}$,
% \begin{align}
%     \mu_i(t) & = \lambda_1 \int_1^t e^{-\lambda_1(t-s)} \nabla_i f(x(s)) ds. \label{eqn:mut}
% \end{align}
% Since $\norm{\nabla f(x(t))}$ is bounded and $\lambda_1> 0$, the above equation implies that $\mu_i(t)$ is bounded.
We consider the possible cases: $\lambda_3 > 0$ and $\lambda_3 = 0$.
\begin{itemize}
    \item $\lambda_3 > 0$ : We can rewrite $\phi_{22}$ as $\phi_{22}(t) = \frac{e^{-\frac{2\lambda_2+\lambda_3-p}{2}t}(p-\lambda_3) + e^{-\frac{2\lambda_2+\lambda_3+p}{2}t}(p+\lambda_3)}{2p}$. Since $p = \sqrt{\lambda_3^2 + 4\lambda_2\lambda_3} < 2\lambda_2+\lambda_3$ and $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded, it follows from~\eqref{eqn:nut} that $\nu_i(t)$ is bounded.
    \item $\lambda_3 = 0$ : In this case, $\nu_i(t) = e^{-\lambda_2 (t-1)} \nu_i(1) + \lambda_2 \int_1^t e^{-\lambda_2 (t-s)} \psi(\nabla_i f(x(s)), \mu_i(s)) d s$. The above implies that $\nu_i(t)$ is bounded as $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded.
\end{itemize}
Earlier, we have shown that $\mu_i(t)$ is bounded and $\nu_i(t) > 0$. From~\eqref{eqn:xm_evol} then we have, $\Dot{x}_i(t)$ is bounded. From~\eqref{eqn:mu_evol} and~\eqref{eqn:xm_evol}, $\mu_i(t) = 0$ implies that $\dot{\mu}_i(t) = \lambda_1 \nabla_i f(x(t))$ and $\dot{x}_i(t) = 0$. Thus, $\mu_i(t)$ can be zero only at isolated points $t$. Otherwise, for some $h>0$ there exists an interval $(t-h,t+h)$ such that $\mu_i(s) = 0$ for all $s \in (t-h,t+h)$. In that case, $\dot{\mu}_i(s) = 0$ for all $s \in (t-h,t+h)$. Since $\dot{\mu}_i(s) = \lambda_1 \nabla_i f(x(s))$ for all $s \in (t-h,t+h)$, we then have $\nabla_i f(x(s)) = 0$ for all $s \in (t-h,t+h)$, which proves the theorem.

We have shown above that $\mu_i(t) = 0$ only at isolated points and $\nu_i(t)$ is bounded. So, $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is bounded except at isolated points.
Since $\mu_i(t)^2 \nu_i(t)^{-0.5}$ is integrable and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is bounded except at isolated points, we have $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is integrable. Since $\nu_i(t)$ is bounded and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is integrable, we have $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-1.5}}$ integrable.
Now, we apply Cauchy-Schwartz inequality on the functions $\mu_i(t) \nu_i(t)^{-0.75} \psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ and $\dfrac{1}{\mu_i(t) \nu_i(t)^{-0.75}}$. Since we have $\mu_i(t)^2 \nu_i(t)^{-1.5} \psi(\nabla_i f(x(t)), \mu_i(t))$ and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-1.5}}$ integrable, the Cauchy-Schwartz inequality implies that $\psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ is integrable. Since $\psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ is bounded and integrable, it is also square-integrable. Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is integrable.

Now, the time-derivative of $\psi$ along the trajectory $x_i(t)$ is
\begin{align*}
    & \dfrac{d}{dt} \psi(\nabla_i f(x(t)), \mu_i(t)) \\
    & = \nabla \psi(\nabla_i f(x(t)), \mu_i(t))^T 
    \begin{bmatrix}
    [\nabla^2 f(x(t))]_i \Dot{x}_i(t) \\ \Dot{\mu}_i(t)
    \end{bmatrix}.
\end{align*}
We have shown that $\nabla_i f(x(t))$ and $\mu_i(t)$ are bounded. Then, according to Assumption~\ref{assump_a}, $\nabla \psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded. From Assumption~\ref{assump_2}, $[\nabla^2 f(x(t))]_i$ is bounded. We have shown that $\Dot{x}_i(t)$ is bounded. Since $\nabla_i f(x(t))$ and $\mu_i(t)$ are bounded,~\eqref{eqn:mu_evol} implies that $\Dot{\mu}_i(t)$ is bounded. Then, from the above equation we have $\dfrac{d}{dt} \psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded. Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is uniformly continuous w.r.t $t$.

We have shown that, for each $i \in \{1,\ldots,d\}$, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is integrable and uniformly continuous. From Barbalat's lemma~\cite{barbalat1959systemes} it follows that $\lim_{t \to \infty} \psi(\nabla_i f(x(t)), \mu_i(t)) = 0$. Then, according to Assumption~\ref{assump_c}, $\lim_{t \to \infty} \nabla_i f(x(t)) = 0$. The proof is complete.
\end{proof}

Now we are ready to show that the Adam and the AdaBelief algorithms are included in our generic adaptive gradient algorithm~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol}. 
The Adam algorithm has been reviewed in Section~\ref{sub:adam}. 
The following two results present convergence of the Adam and the AdaBelief algorithm in continuous-time. Specifically, we obtain the following corollaries of Theorem~\ref{thm:gen}.

\begin{corollary} \label{cor:adam}
Consider the set of differential equations~\eqref{eqn:mu_adam}-\eqref{eqn:xm_adam} with initial conditions $\mu(1) = 0_d$, $x(1) \in \R^d$, and $\{v_i(1) > 0 : i = 1,\ldots,d\}$. Let the parameters $\lambda_1$ and $\lambda_2$ satisfy $0 < \lambda_2 < \lambda_1 < 1$. If Assumptions~\ref{assump_1}-\ref{assump_2} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{corollary}

\begin{proof}
The set of equations~\eqref{eqn:mu_adam}-\eqref{eqn:xm_adam} is a special case of~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with $\lambda_3 = 0$ and $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$. Clearly, $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$ satisfies Assumption~\ref{assump_3}. Thus, Theorem~\ref{thm:gen} is applicable, and the proof follows.
\end{proof}

\begin{corollary} \label{cor:adabelief}
Consider the set of differential equations~\eqref{eqn:mu_adabelief}-\eqref{eqn:xm_adabelief} with initial conditions $\mu(1) = 0_d$, $x(1) \in \R^d$, and $\{v_i(1) > 0 : i = 1,\ldots,d\}$. Let the parameters $\lambda_1$ and $\lambda_2$ satisfy $0 < \lambda_2 < \lambda_1 < 1$. If Assumptions~\ref{assump_1}-\ref{assump_2} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{corollary}

\begin{proof}
The set of equations~\eqref{eqn:mu_adabelief}-\eqref{eqn:xm_adabelief} is a special case of~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with $\lambda_3 = 0$ and $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))-\mu_i(t)}^2$. Clearly, $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))-\mu_i(t)}^2$ satisfies Assumption~\ref{assump_a}-\ref{assump_b}. We will show that it also satisfies Assumption~\ref{assump_c}.

Suppose that $\lim_{t \to \infty} \norm{\nabla_i f(x(t))-\mu_i(t)}^2 = 0$. Then, $\lim_{t \to \infty} \nabla_i f(x(t)) = \lim_{t \to \infty} \mu_i(t)$. We define $\mu_i^* = \lim_{t \to \infty} \nabla_i f(x(t)) = \lim_{t \to \infty} \mu_i(t)$. We claim that $\mu_i^* = 0$. Otherwise, suppose that $\mu_i^* \neq 0$. Then, there exists $T < \infty$ such that $\mu_i(t)$ and $\nabla_i f(x(t))$ have the same sign for all $t \geq T$. Then, from~\eqref{eqn:fdot_2}, $\Dot{f}(x(t)) < 0$ for all $t \geq T$. Since $f$ is bounded below, due to Assumption~\eqref{assump_1}, and decreasing for all $t \geq T$, $f(x(t))$ converges to its minimum value as $t \to \infty$. From first order optimality condition, then we have $\lim_{t \to \infty} \nabla f(x(t)) = 0$. So, $\mu_i^* = 0$, which is a contradiction. Thus, Assumption~\ref{assump_c} holds and the proof is complete following Theorem~\ref{thm:gen}.
\end{proof}



























==> general_new.tex <==
\section{A Generic Adaptive Gradient Algorithm}
\label{sec:gen}

In this section, we propose a generic adaptive gradient algorithm and create a state-space framework for analyzing Adam-like adaptive gradient algorithms. 
% and inspired by the analysis of G-AdaGrad algorithm, as presented in the proof of Theorem~\ref{thm:adagrad}.

We make the following assumptions in order to present the algorithms in this paper and their convergence results.

\begin{assumption} \label{assump_1}
Assume that the minimum of function $f$ exists and is finite, i.e., $\mnorm{\min_{x \in \R^d} f(x)} < \infty$.
\end{assumption}

\begin{assumption} \label{assump_2}
Assume that $f$ is twice differentiable over its domain $\R^d$ and the entries in the Hessian matrix $\nabla^2 f(x)$ are bounded for all $x\in \R^d$.
\end{assumption}

The above assumptions are mild and standard in the literature of gradient-based optimization. Assumption~\ref{assump_1} implies that the optimization problem~\eqref{eqn:opt_1} has a solution. Assumption~\ref{assump_2} is equivalent to the gradient $\nabla f$ being Lipschitz continuous, which is also referred as the function $f$ being {\em smooth}~\cite{ZaheerRSKK18, de2018convergence}.

Our framework of adaptive gradient algorithms hinges on their state-space representation in terms of ODEs. The proposed generic adaptive gradient algorithm is similar to the Adam method described in Section~\ref{sub:adam}. However, there are two notable differences.
\begin{itemize}
    \item Firstly, we replace the squared-gradient term $\norm{\nabla_i f(x(t))}^2$ in the evolution of second raw moment estimate in~\eqref{eqn:v_adam} with $\psi(\nabla_i f(x(t)), \mu_i(t))$, where we define $\psi$ as an well-behaved and non-negative valued function $\psi:\R^2 \to \R_{\geq 0}$. The sufficient conditions on the general function $\psi$ which guarantees convergence of the generic algorithm are specified later in this section. Needless to say, the generic setup includes the original Adam algorithm, i.e., $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$, as a special case.
    \item The other difference is that, in our algorithm, the ODE governing the second raw moment estimate of the gradients has a higher order. An issue with the Adam algorithm is that the ODEs~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} for the first and second moments can converge slowly, especially if the optimization problem~\eqref{eqn:opt_1} is ill-conditioned, leading to a slower convergence of the estimate. Now, each of the ODEs~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} can be seen as a controlled linear-time invariant (LTI) system. The controlled inputs for~\eqref{eqn:mu_adam}-\eqref{eqn:v_adam} are, respectively, $\nabla_i f(x(t))$ and $\norm{\nabla_i f(x(t))}^2$. It is known that addition of a zero improves the transient response of an LTI system. Note that, the Adam algorithm does not have any zero in the dynamics~\eqref{eqn:v_adam}. So, in our algorithm, we add a left-half plane zero to the dynamics in~\eqref{eqn:v_adam} for improving the convergence rate. However, in the Adam algorithm, the dynamics in~\eqref{eqn:v_adam} is {\em strictly proper}. Thus, we also add an additional left half-plane pole in~\eqref{eqn:v_adam}. Hence, for each dimension $i \in \{1,\ldots,d\}$, the transfer function from $\psi(\nabla_i f(x(t)), \mu_i(t))$ to the second raw moment estimate $\nu_i(t)$ in our generic setup has an additional pole-zero pair in the left-half plane, as compared to only one pole and no zero for its counterpart in the Adam method. Herein lies the intuition behind our algorithm.
\end{itemize}

% We demonstrate this with the following numerical example. In this example, we consider the classification task of handwritten digits one and five, using the MNIST~\cite{} dataset. We consider the logistic regression model and conduct experiments for minimizing the cross-entropy error on the training data. 

Our generic adaptive gradient algorithm is iterative in nature where, at each time $t\geq 1$, it maintains four $d$-dimensional vectors: an estimate $x(t)$ of a minimum point of~\eqref{eqn:opt_1}, an estimate $\mu(t)$ of the first moment of gradients, an estimate $\nu(t)$ of the second raw moment of gradients, and an additional $\zeta(t)$ due to higher order of the transfer functions from $\psi(\nabla_i f(x(t)), \mu_i(t))$ to $\nu_i(t)$. The initial estimate $x(1)$ is chosen arbitrarily from $\R^d$. The variables $\mu$ and $\zeta$ are initialized at $t=1$ as the $d$-dimensional zero vector, denoted by $0_d$. The remaining variable $\nu$ is initialized according to $\{\nu_i(0) > 0 : i = 1,\ldots,d\}$. Before initiating the iterative process, the algorithm chooses eight non-negative real-valued scalar parameters $\lambda_1,\ldots,\lambda_8$. Their specific conditions are presented later in this section. Given the parameters $\lambda_2 \in (0,1)$ and $\lambda_6 \in (0,1)$, we define a positive-valued function $\alpha_g: [0,\infty) \to \R$ by
\begin{align}
    \alpha_g(t) &=
    \begin{cases}
    \dfrac{1-(1-\lambda_2)^{t+1}}{\sqrt{1-(1-\lambda_6)^{t+1}}}, & \text{if } \lambda_7 > 0 \\
    1, &  \text{if } \lambda_7 = 0. \label{eqn:alpha_g}
    \end{cases}
\end{align}
For time $t\geq 0$, the algorithm steps in continuous-time domain are governed by the following set of ODEs
\begin{align}
    \Dot{\mu}_i(t) & = -\lambda_1 \mu_i(t) + \lambda_2 \nabla_i f(x(t)), \label{eqn:mu_evol} \\
    \Dot{\zeta}_i(t) & = -\lambda_3 \zeta_i(t) + \lambda_3 \nu_i(t), \label{eqn:z_evol} \\
    \Dot{\nu}_i(t) & = \lambda_4 \zeta_i(t) - \lambda_5 \nu_i(t) + \lambda_6 \psi(\nabla_i f(x(t)), \mu_i(t)), \label{eqn:nu_evol} \\
    \Dot{x}_i(t) & = - \dfrac{1}{\alpha_g(t)} \dfrac{\lambda_7 \mu_i(t) + \lambda_8 \nabla_i f(x(t))}{\sqrt{\nu_i(t)}}. \label{eqn:xm_evol}
\end{align}
The $d$-dimensional vectors $\mu$, $\zeta$, and $\nu$ can be abstracted as dynamic controller states. Here, $\alpha_g(t)$ represents the initial bias correction. When the moment estimate is not used in updating $x(t)$, there is no bias correction needed in the algorithm, e.g. AdaGrad~\cite{duchi2011adaptive}. Such cases are represented by $\lambda_7 = 0$ and $\alpha_g(t) = 1$ because of no bias correction.

\begin{assumption} \label{assump_3}
We assume that the function $\psi$ satisfies the following properties.
\begin{enumerate}[label={\textbf{\Alph*:}},
  ref={\theassumption.\Alph*}]
    \item $\psi$ is differentiable over $\R^2$. Moreover, $\psi(x,y)$ and its gradient $\nabla \psi (x,y)$ are bounded if both $x$ and $y$ are bounded, for any $x,y \in \R$. \label{assump_a}
    \item $\psi(x,.)$ is bounded only if $x$ is bounded, for $x \in \R$. \label{assump_b}
    \item $\lim_{t \to \infty} \psi(\nabla_i f(x(t)), \mu_i(t)) = 0$ only if $\lim_{t \to \infty} \nabla_i f(x(t)) = 0$. \label{assump_c}
\end{enumerate}
\end{assumption}

Assumption~\ref{assump_a} implies that the function $\psi$ is smooth enough. Assumption~\ref{assump_b} means that $\psi$ is radially unbounded in its first argument.

The following theorem guarantees convergence of our generic adaptive gradient algorithm, presented above in~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol}, to a critical point of problem~\eqref{eqn:opt_1}.

\begin{theorem} \label{thm:gen}
Consider the set of differential equations~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with initial conditions $\mu(0) = \zeta(0) = 0_d$, $x(0) \in \R^d$, and $\{v_i(0) > 0 : i = 1,\ldots,d\}$. Let the parameters satisfy
\begin{align}
    0 < \lambda_6 < \lambda_2 < 1, \, \lambda_3 > 0, \, \lambda_4 \geq 0, \, \lambda_4 < \lambda_5 < 4\lambda_1, \nonumber \\
    \lambda_6 > 0, \, \lambda_7 \geq 0, \, \lambda_8 \geq 0, \lambda_7\lambda_8 > 0. \label{eqn:lambda_cond}
\end{align}
If Assumptions~\ref{assump_1}-\ref{assump_3} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{theorem}


\begin{proof}
The time-derivative of $f$ along the trajectories $x(t)$  of~\eqref{eqn:xm_evol} is given by
\begin{align}
    & \Dot{f}(x(t)) = \sum_{i=1}^d \nabla_i f(x(t)) \Dot{x}_{i}(t) \nonumber \\
    &= - \sum_{i=1}^d \dfrac{1}{\alpha_g(t)} \dfrac{\lambda_7 \nabla_i f(x(t)) \mu_i(t) + \lambda_8 \norm{\nabla_i f(x(t))}^2}{\sqrt{\nu_i(t)}}. \label{eqn:fdot_2}
\end{align}
Upon multiplying with $\alpha_g(t)$ on both sides above, followed by integrating both sides w.r.t. $s$ from $1$ to $t$ and substituting from~\eqref{eqn:mu_evol} we have
\begin{align}
    & \int_0^t \alpha_g(s)\Dot{f}(x(s))ds = - \sum_{i=1}^d \int_0^t \dfrac{\lambda_7\mu_i(s)\Dot{\mu}_i(s)}{\lambda_2 \sqrt{\nu_i(s)}}ds \nonumber\\
    & - \sum_{i=1}^d \int_0^t \dfrac{\lambda_7\lambda_1\mu_i(s)^2}{\lambda_2\sqrt{\nu_i(s)}}ds - \sum_{i=1}^d \int_0^t \dfrac{\lambda_8\norm{\nabla_i f(x(s))}^2}{\sqrt{\nu_i(s)}}ds. \label{eqn:total_int}
\end{align}
Integrating by parts we have the first term on R.H.S. as
\begin{align*}
    & \int_0^t \dfrac{\mu_i(s)\Dot{\mu}_i(s)}{\sqrt{\nu_i(s)}}ds
    = \left[\dfrac{\mu_i(s)^2}{2\sqrt{\nu_i(s)}}\right]_1^t + \dfrac{1}{4} \int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \Dot{\nu}_i(s) ds.
\end{align*}
Upon substituting above from~\eqref{eqn:nu_evol}, and using that $\mu(0)=0_d$,
\begin{align*}
    & \int_0^t \dfrac{\mu_i(s)\Dot{\mu}_i(s)}{\sqrt{\nu_i(s)}}ds
    = \dfrac{\mu_i(t)^2}{2\sqrt{\nu_i(t)}} + \dfrac{\lambda_4}{4} \int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \\
    & - \dfrac{\lambda_5}{4}\int_0^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \\
    & + \dfrac{\lambda_6}{4}\int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds.
\end{align*}
Upon substituting above in~\eqref{eqn:total_int} we obtain that
\begin{align}
    & \int_0^t \alpha_g(s)\Dot{f}(x(s))ds
    = - \sum_{i=1}^d \dfrac{\lambda_7\mu_i(t)^2}{2\lambda_2\sqrt{\nu_i(t)}} \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7\lambda_4}{4\lambda_2} \int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7}{\lambda_2} \left(\lambda_1-\dfrac{\lambda_5}{4}\right)\int_0^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7\lambda_6}{4\lambda_2}\int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds \nonumber \\
    & - \sum_{i=1}^d \int_0^t \dfrac{\lambda_8\norm{\nabla_i f(x(s))}^2}{\sqrt{\nu_i(s)}}ds. \label{eqn:int_expand}
\end{align}

We consider the possible cases $\lambda_7 = 0$ and $\lambda_7 > 0$. First we consider $\lambda_7 = 0$. In this case, $\alpha_g(t) = 1$ (see~\eqref{eqn:alpha_g}). From~\eqref{eqn:alphaV},
\begin{align*}
    f(x(t)) = - \sum_{i=1}^d \int_0^t \dfrac{\lambda_8\norm{\nabla_i f(x(s))}^2}{\sqrt{\nu_i(s)}}ds.
\end{align*}
Since $\lambda_8 > 0$, the above implies that $f(x(t))$ is decreasing in $t$. From Assumption~\ref{assump_1}, then it follows that $\lim_{t \to \infty} f(x(t)) = \min_{x \in \R^d} f(x)$. By first order necessary condition of optimality, then we have $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$. In the remainder of the proof, we consider the case $\lambda_7 > 0$.

We define, $\gamma_1 = 1-\lambda_2$ and $\gamma_2 = 1-\lambda_6$.
Upon differentiating both sides of~\eqref{eqn:alpha_g} w.r.t $t$ we get $\Dot{\alpha_g}(t) = \dfrac{\gamma_2^{t+1}(1-\gamma_1^{t+1})\log{\gamma_2} - 2\gamma_1^{t+1}(1-\gamma_2^{t+1})\log{\gamma_1}}{2(1-\gamma_2^{t+1})^{1.5}}$.
So we have
\begin{align}
    \Dot{\alpha_g}(t) < 0 \iff \left(\dfrac{\gamma_2}{\gamma_1}\right)^{t+1} \dfrac{1-\gamma_1^{t+1}}{1-\gamma_2^{t+1}} > 2\dfrac{\log{\gamma_1}}{\log{\gamma_2}}. \label{eqn:cond}
\end{align}
From the condition $\lambda_2 > \lambda_6$ in~\eqref{eqn:lambda_cond}, we have $1 > \gamma_2 > \gamma_1 > 0$. Then, $\left(\dfrac{\gamma_2}{\gamma_1}\right)^{t+1}$ and $\dfrac{1-\gamma_1^{t+1}}{1-\gamma_2^{t+1}}$ are, respectively, increasing and decreasing functions of $t$. Since $1 > \gamma_2 > \gamma_1 > 0$, we have $\lim_{t \to \infty} \left(\dfrac{\gamma_2}{\gamma_1}\right)^t \to \infty$ and $\lim_{t \to \infty} \dfrac{1-\gamma_1^t}{1-\gamma_2^t} = 1$. Thus, $\left(\dfrac{\gamma_2}{\gamma_1}\right)^t \dfrac{1-\gamma_1^t}{1-\gamma_2^t}$ is an increasing function of $t$. Then, there exists $T < \infty$ such that~\eqref{eqn:cond} holds for all $t \geq T$. 
Integrating by parts we rewrite the L.H.S. in~\eqref{eqn:int_expand} as
\begin{align*}
    & \int_0^t \alpha_g(s)\Dot{f}(x(s))ds = \left[\alpha_g(s)f(x(s))\right]_0^t - \int_0^t \Dot{\alpha_g}(s)f(x(s))ds.
\end{align*}
Upon substituting from above in~\eqref{eqn:int_expand}, for $t \geq T$,
\begin{align}
    & \alpha_g(t)f(x(t)) + \sum_{i=1}^d \dfrac{\lambda_7\mu_i(t)^2}{2\lambda_2\sqrt{\nu_i(t)}} = \alpha_g(0)f(x(0)) \nonumber \\
    & + \int_0^{T} \Dot{\alpha_g}(s)f(x(s))ds + \int_{T}^t \Dot{\alpha_g}(s)f(x(s))ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7\lambda_4}{4\lambda_2} \int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \zeta_i(s) ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7}{\lambda_2} \left(\lambda_1-\dfrac{\lambda_5}{4}\right)\int_0^t \mu_i(s)^2 \nu_i(s)^{-0.5} ds \nonumber \\
    & - \sum_{i=1}^d \dfrac{\lambda_7\lambda_6}{4\lambda_2}\int_0^t \mu_i(s)^2 \nu_i(s)^{-1.5} \psi(\nabla_i f(x(s)), \mu_i(s)) ds \nonumber \\
    & - \sum_{i=1}^d \int_0^t \dfrac{\lambda_8\norm{\nabla_i f(x(s))}^2}{\sqrt{\nu_i(s)}}ds. \label{eqn:alphaV}
\end{align}

For each $i \in \{1,\ldots,d\}$, consider the LTI system described by~\eqref{eqn:z_evol}-\eqref{eqn:nu_evol}, with the state vector $[\zeta_i,\nu_i]^T \in \R^2$. From~\eqref{eqn:lambda_cond}, $\lambda_4 \geq 0$. Here, we consider the possible cases: $\lambda_4 > 0$ and $\lambda_4 = 0$.
\begin{itemize}
    \item $\lambda_4 > 0$ : Define the state matrix $A = \begin{bmatrix} -\lambda_3 & \lambda_3 \\ \lambda_4 & -\lambda_5 \end{bmatrix}$. Since $\zeta(1) = 0_d$, the states are given by the solution
\begin{align*}
    \begin{bmatrix} \zeta_i(t) \\ \nu_i(t) \end{bmatrix} & = e^{A t} \begin{bmatrix} 0 \\ \nu_i(0)\end{bmatrix} \\ & + \int_0^t e^{A (t-s)} \begin{bmatrix} 0 \\ \lambda_6 \end{bmatrix} \psi(\nabla_i f(x(s)), \mu_i(s)) d s.
\end{align*}
Upon computing the state-transition matrix $e^{A t}$ and substituting above, we obtain that
\begin{align}
    \zeta_i(t) & = \phi_{12}(t) \nu_i(0) \nonumber \\ & + \lambda_6 \int_0^t \phi_{12}(t-s) \psi(\nabla_i f(x(s)), \mu_i(s)) d s, \label{eqn:zt} \\
    \nu_i(t) & = \phi_{22}(t) \nu_i(0) \nonumber \\ & + \lambda_6 \int_0^t \phi_{22}(t-s) \psi(\nabla_i f(x(s)), \mu_i(s)) d s, \label{eqn:nut}
\end{align}
where $\phi_{12}(t) = \lambda_3 e^{-\frac{\lambda_3+\lambda_5}{2}t} \frac{e^{\frac{p}{2}t}-e^{-\frac{p}{2}t}}{p}$, $\phi_{22}(t) = e^{-\frac{\lambda_3+\lambda_5}{2}t} \frac{e^{\frac{p}{2}t}(p-\lambda_5+\lambda_3) + e^{-\frac{p}{2}t}(p+\lambda_5-\lambda_3)}{2p}$, and $p = \sqrt{(\lambda_3-\lambda_5)^2 + 4\lambda_3\lambda_4}$. Since $\lambda_3,\lambda_6 > 0$ (ref.~\eqref{eqn:lambda_cond}), $\nu_i(0) > 0$, $\psi \geq 0$, and $p > 0$, from~\eqref{eqn:zt} we have $\zeta_i(t) > 0$. Since $\lambda_3, \lambda_4 > 0$, we have $p = \sqrt{(\lambda_3-\lambda_5)^2 + 4\lambda_3\lambda_4} > |\lambda_5-\lambda_3|$, which implies that $\phi_{22}(t) > 0$. From above and $\nu_i(0) > 0$, we have $\nu_i(t) > 0$.
    \item $\lambda_4 = 0$ : From~\eqref{eqn:nu_evol}, $\Dot{\nu}_i(t) = - \lambda_5 \nu_i(t) + \lambda_6 \psi(\nabla_i f(x(t)), \mu_i(t))$. The solution of this ODE is $\nu_i(t) = e^{-\lambda_5 t} \nu_i(0) + \lambda_6 \int_0^t e^{-\lambda_5 (t-s)} \psi(\nabla_i f(x(s)), \mu_i(s)) d s$, which implies that $\nu_i(t) > 0$.
\end{itemize}

Since $\zeta_i(t) > 0$ and $\psi \geq 0$, due to~\eqref{eqn:lambda_cond} and~\eqref{eqn:cond}, the R.H.S. in~\eqref{eqn:alphaV} is decreasing in $t \geq T$. Then, the L.H.S. in~\eqref{eqn:alphaV} is also decreasing in $t \geq T$. Since $\mu_i(t)$ and $\nu_i(t)$ are continuous and $\nu_i(t) > 0$, $\dfrac{\lambda_7\mu_i(t)^2}{2\lambda_2\sqrt{\nu_i(t)}}$ is continuous. Also, $\alpha_g(t)f(x(t))$ is continuous. Thus, considering the compact interval $[1,T]$, $\alpha_g(T)f(x(T)) + \sum_{i=1}^d \dfrac{\lambda_7\mu_i(T)^2}{2\lambda_2\sqrt{\nu_i(T)}} =: M_T$ is finite. Since the L.H.S. in~\eqref{eqn:alphaV} is decreasing in $t \geq T$, we have the L.H.S. in~\eqref{eqn:alphaV} bounded above by $M_T$ for all $t \geq T$. 

From the R.H.S. of~\eqref{eqn:alphaV} then we have that $\mu_i(t)^2 \nu_i(t)^{-1.5} \psi(\nabla_i f(x(t)), \mu_i(t))$ and $\mu_i(t)^2 \nu_i(t)^{-0.5}$ are integrable w.r.t. $t$ and bounded. Thus, $\mu_i(t)$ is bounded. Moreover, if $\lambda_8 > 0$, we also have $\dfrac{\norm{\nabla_i f(x(t))}^2}{\sqrt{\nu_i(t)}}$ integrable and bounded. It implies that, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded unless $\mu_i(t) = 0$ or $\nu_i(t) = \infty$. To show that $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded even if $\mu_i(t) = 0$ or $\nu_i(t) = \infty$, we consider the possible cases: $\lambda_8 = 0$ and $\lambda_8 > 0$.
\begin{itemize}
    \item $\lambda_8 = 0$ : From~\eqref{eqn:xm_evol}, either of the conditions $\mu_i(t) = 0$ and $\nu_i(t) = \infty$ implies that $\dot{x}_i(t) = 0$ and, hence, $\frac{d}{dt}\nabla_i f(x(t)) = 0$. Due to continuity of $\nabla_i f$, we then have $\nabla_i f(x(t))$ is bounded. From Assumption~\ref{assump_a}, $\nabla_i f(x(t))$ and $\mu_i(t)$ being bounded implies that $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded.  
    \item $\lambda_8 = 0$ : In this case, $\dfrac{\norm{\nabla_i f(x(t))}^2}{\sqrt{\nu_i(t)}}$ is bounded. Thus, $\nabla_i f(x(t))$ is bounded unless $\nu_i(t) = \infty$, in which case $\dot{x}_i(t) = 0$. Following the argument in the previous case, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded. 
\end{itemize}
Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded, and therefore, Assumption~\ref{assump_b} implies that $\nabla_i f(x(t))$ is bounded.



% Integrating both sides of~\eqref{eqn:mu_evol} w.r.t $t$ from $1$ to $t$, we have for $i \in \{1,\ldots,d\}$,
% \begin{align}
%     \mu_i(t) & = \lambda_1 \int_0^t e^{-\lambda_1(t-s)} \nabla_i f(x(s)) ds. \label{eqn:mut}
% \end{align}
% Since $\norm{\nabla f(x(t))}$ is bounded and $\lambda_1> 0$, the above equation implies that $\mu_i(t)$ is bounded.
To show that $\nu_i(t)$ is bounded, we consider the possible cases: $\lambda_4 > 0$ and $\lambda_4 = 0$.
\begin{itemize}
    \item $\lambda_4 > 0$ : We can rewrite $\phi_{22}$ as $\phi_{22}(t) = \frac{e^{-\frac{\lambda_3+\lambda_5-p}{2}t}(p-\lambda_5+\lambda_3) + e^{-\frac{\lambda_3+\lambda_5+p}{2}t}(p+\lambda_5-\lambda_3)}{2p}$. Since $p = \sqrt{(\lambda_3-\lambda_5)^2 + 4\lambda_3\lambda_4} < \lambda_3+\lambda_5$ for $\lambda_5 > \lambda_4$ (see~\eqref{eqn:lambda_cond}) and $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded, it follows from~\eqref{eqn:nut} that $\nu_i(t)$ is bounded.
    \item $\lambda_4 = 0$ : In this case, $\nu_i(t) = e^{-\lambda_5 t} \nu_i(0) + \lambda_6 \int_0^t e^{-\lambda_5 (t-s)} \psi(\nabla_i f(x(s)), \mu_i(s)) d s$. The above implies that $\nu_i(t)$ is bounded as $\psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded.
\end{itemize}
Earlier, we have shown that $\mu_i(t)$ is bounded and $\nu_i(t) > 0$. From~\eqref{eqn:xm_evol} then we have, $\Dot{x}_i(t)$ is bounded. From~\eqref{eqn:mu_evol}, $\mu_i(t) = 0$ implies that $\dot{\mu}_i(t) = \lambda_1 \nabla_i f(x(t))$. Thus, $\mu_i(t)$ can be zero only at isolated points $t$. Otherwise, for some $h>0$ there exists an interval $(t-h,t+h)$ such that $\mu_i(s) = 0$ for all $s \in (t-h,t+h)$. In that case, $\dot{\mu}_i(s) = 0$ for all $s \in (t-h,t+h)$. Since $\dot{\mu}_i(s) = \lambda_1 \nabla_i f(x(s))$ for all $s \in (t-h,t+h)$, we then have $\nabla_i f(x(s)) = 0$ for all $s \in (t-h,t+h)$, which proves the theorem.

We have shown above that $\mu_i(t) = 0$ only at isolated points and $\nu_i(t)$ is bounded. So, $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is bounded except at isolated points.
Since $\mu_i(t)^2 \nu_i(t)^{-0.5}$ is integrable and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is bounded except at isolated points, we have $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is integrable. Since $\nu_i(t)$ is bounded and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-0.5}}$ is integrable, we have $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-1.5}}$ integrable.
Now, we apply Cauchy-Schwartz inequality on the functions $\mu_i(t) \nu_i(t)^{-0.75} \psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ and $\dfrac{1}{\mu_i(t) \nu_i(t)^{-0.75}}$. Since we have $\mu_i(t)^2 \nu_i(t)^{-1.5} \psi(\nabla_i f(x(t)), \mu_i(t))$ and $\dfrac{1}{\mu_i(t)^2 \nu_i(t)^{-1.5}}$ integrable, the Cauchy-Schwartz inequality implies that $\psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ is integrable. Since $\psi(\nabla_i f(x(t)), \mu_i(t))^{0.5}$ is bounded and integrable, it is also square-integrable. Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is integrable.

Now, the time-derivative of $\psi$ along the trajectory $x_i(t)$ is
\begin{align*}
    & \dfrac{d}{dt} \psi(\nabla_i f(x(t)), \mu_i(t)) \\
    & = \nabla \psi(\nabla_i f(x(t)), \mu_i(t))^T 
    \begin{bmatrix}
    [\nabla^2 f(x(t))]_i \Dot{x}_i(t) \\ \Dot{\mu}_i(t)
    \end{bmatrix}.
\end{align*}
We have shown that $\nabla_i f(x(t))$ and $\mu_i(t)$ are bounded. Then, according to Assumption~\ref{assump_a}, $\nabla \psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded. From Assumption~\ref{assump_2}, $[\nabla^2 f(x(t))]_i$ is bounded. We have shown that $\Dot{x}_i(t)$ is bounded. Since $\nabla_i f(x(t))$ and $\mu_i(t)$ are bounded,~\eqref{eqn:mu_evol} implies that $\Dot{\mu}_i(t)$ is bounded. Then, from the above equation we have $\dfrac{d}{dt} \psi(\nabla_i f(x(t)), \mu_i(t))$ is bounded. Thus, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is uniformly continuous w.r.t $t$.

We have shown that, for each $i \in \{1,\ldots,d\}$, $\psi(\nabla_i f(x(t)), \mu_i(t))$ is integrable and uniformly continuous. From Barbalat's lemma~\cite{barbalat1959systemes} it follows that $\lim_{t \to \infty} \psi(\nabla_i f(x(t)), \mu_i(t)) = 0$. Then, according to Assumption~\ref{assump_c}, $\lim_{t \to \infty} \nabla_i f(x(t)) = 0$. The proof is complete.
\end{proof}

Now we are ready to show that the Adam and the AdaBelief algorithms are included in our generic adaptive gradient algorithm~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol}. 
The Adam algorithm has been reviewed in Section~\ref{sub:adam}. 
The following two results present convergence of the Adam and the AdaBelief algorithm in continuous-time. Specifically, we obtain the following corollaries of Theorem~\ref{thm:gen}.

\begin{corollary} \label{cor:adam}
Consider the set of differential equations~\eqref{eqn:mu_adam}-\eqref{eqn:xm_adam} with initial conditions $\mu(0) = 0_d$, $x(1) \in \R^d$, and $\{v_i(1) > 0 : i = 1,\ldots,d\}$. Let the parameters $\lambda_1$ and $\lambda_2$ satisfy $0 < \lambda_2 < \lambda_1 < 1$. If Assumptions~\ref{assump_1}-\ref{assump_2} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{corollary}

\begin{proof}
The set of equations~\eqref{eqn:mu_adam}-\eqref{eqn:xm_adam} is a special case of~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with $\lambda_3 = 0$ and $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$. Clearly, $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))}^2$ satisfies Assumption~\ref{assump_3}. Thus, Theorem~\ref{thm:gen} is applicable, and the proof follows.
\end{proof}

\begin{corollary} \label{cor:adabelief}
Consider the set of differential equations~\eqref{eqn:mu_adabelief}-\eqref{eqn:xm_adabelief} with initial conditions $\mu(0) = 0_d$, $x(1) \in \R^d$, and $\{v_i(1) > 0 : i = 1,\ldots,d\}$. Let the parameters $\lambda_1$ and $\lambda_2$ satisfy $0 < \lambda_2 < \lambda_1 < 1$. If Assumptions~\ref{assump_1}-\ref{assump_2} hold, then $\lim_{t \to \infty} \nabla f(x(t)) = 0_d$.
\end{corollary}

\begin{proof}
The set of equations~\eqref{eqn:mu_adabelief}-\eqref{eqn:xm_adabelief} is a special case of~\eqref{eqn:mu_evol}-\eqref{eqn:xm_evol} with $\lambda_3 = 0$ and $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))-\mu_i(t)}^2$. Clearly, $\psi(\nabla_i f(x(t)), \mu_i(t)) = \norm{\nabla_i f(x(t))-\mu_i(t)}^2$ satisfies Assumption~\ref{assump_a}-\ref{assump_b}. We will show that it also satisfies Assumption~\ref{assump_c}.

Suppose that $\lim_{t \to \infty} \norm{\nabla_i f(x(t))-\mu_i(t)}^2 = 0$. Then, $\lim_{t \to \infty} \nabla_i f(x(t)) = \lim_{t \to \infty} \mu_i(t)$. We define $\mu_i^* = \lim_{t \to \infty} \nabla_i f(x(t)) = \lim_{t \to \infty} \mu_i(t)$. We claim that $\mu_i^* = 0$. Otherwise, suppose that $\mu_i^* \neq 0$. Then, there exists $T < \infty$ such that $\mu_i(t)$ and $\nabla_i f(x(t))$ have the same sign for all $t \geq T$. Then, from~\eqref{eqn:fdot_2}, $\Dot{f}(x(t)) < 0$ for all $t \geq T$. Since $f$ is bounded below, due to Assumption~\eqref{assump_1}, and decreasing for all $t \geq T$, $f(x(t))$ converges to its minimum value as $t \to \infty$. From first order optimality condition, then we have $\lim_{t \to \infty} \nabla f(x(t)) = 0$. So, $\mu_i^* = 0$, which is a contradiction. Thus, Assumption~\ref{assump_c} holds and the proof is complete following Theorem~\ref{thm:gen}.
\end{proof}


























